Boosting as Frank-Wolfe

Some boosting algorithms, such as LPBoost, ERLPBoost, and C-ERLPBoost, aim to solve the soft margin optimization problem with the $\ell_1$-norm regularization. LPBoost rapidly converges to an $\epsilon$-approximate solution in practice, but it is known to take $\Omega(m)$ iterations in the worst case, where $m$ is the sample size. On the other hand, ERLPBoost and C-ERLPBoost are guaranteed to converge to an $\epsilon$-approximate solution in $O(\frac{1}{\epsilon^2} \ln \frac{m}{\nu})$ iterations. However, the computation per iteration is very high compared to LPBoost. To address this issue, we propose a generic boosting scheme that combines the Frank-Wolfe algorithm and any secondary algorithm and switches one to the other iteratively. We show that the scheme retains the same convergence guarantee as ERLPBoost and C-ERLPBoost. One can incorporate any secondary algorithm to improve in practice. This scheme comes from a unified view of boosting algorithms for soft margin optimization. More specifically, we show that LPBoost, ERLPBoost, and C-ERLPBoost are instances of the Frank-Wolfe algorithm. In experiments on real datasets, one of the instances of our scheme exploits the better updates of the secondary algorithm and performs comparably with LPBoost.

==> table/test.tex <==
\begin{tabular}{lrrr}
    \toprule
	         &            LPB. &          ERLPB. &      MLPB. (SS) \\ \midrule \addlinespace[0.5em]
	Banana   & 0.14 $\pm$ 0.01 & 0.15 $\pm$ 0.01 & 0.14 $\pm$ 0.01 \\          \addlinespace[0.5em]
	B.Cancer & 0.32 $\pm$ 0.05 & 0.32 $\pm$ 0.05 & 0.33 $\pm$ 0.04 \\          \addlinespace[0.5em]
	Diabetes & 0.30 $\pm$ 0.02 & 0.30 $\pm$ 0.02 & 0.30 $\pm$ 0.02 \\          \addlinespace[0.5em]
	F.Solar  & 0.44 $\pm$ 0.02 & 0.45 $\pm$ 0.06 & 0.34 $\pm$ 0.01 \\          \addlinespace[0.5em]
	German   & 0.27 $\pm$ 0.03 & 0.28 $\pm$ 0.02 & 0.27 $\pm$ 0.02 \\          \addlinespace[0.5em]
	Heart    & 0.22 $\pm$ 0.04 & 0.23 $\pm$ 0.04 & 0.23 $\pm$ 0.04 \\          \addlinespace[0.5em]
	Image    & 0.03 $\pm$ 0.01 & 0.03 $\pm$ 0.01 & 0.03 $\pm$ 0.01 \\          \addlinespace[0.5em]
	Ringnorm & 0.12 $\pm$ 0.01 & 0.13 $\pm$ 0.01 & 0.13 $\pm$ 0.01 \\          \addlinespace[0.5em]
	Splice   & 0.05 $\pm$ 0.01 & 0.05 $\pm$ 0.00 & 0.04 $\pm$ 0.01 \\          \addlinespace[0.5em]
	Thyroid  & 0.09 $\pm$ 0.04 & 0.09 $\pm$ 0.03 & 0.08 $\pm$ 0.03 \\          \addlinespace[0.5em]
	Titanic  & 0.66 $\pm$ 0.05 & 0.60 $\pm$ 0.12 & 0.22 $\pm$ 0.01 \\          \addlinespace[0.5em]
	Twonorm  & 0.05 $\pm$ 0.00 & 0.05 $\pm$ 0.00 & 0.05 $\pm$ 0.00 \\          \addlinespace[0.5em]
	Waveform & 0.12 $\pm$ 0.01 & 0.12 $\pm$ 0.01 & 0.12 $\pm$ 0.01 \\          \addlinespace[0.5em]
    \bottomrule
\end{tabular}
